Applications of the Feynman-Hellmann theorem in hadron structure

The Feynman-Hellmann (FH) relation offers an alternative way of accessing hadronic matrix elements through artificial modifications to the QCD Lagrangian. In particular, a FH-motivated method provides a new approach to calculations of disconnected contributions to matrix elements and high-momentum nucleon and pion form factors. Here we present results for the total nucleon axial charge, including a statistically significant non-negative total disconnected quark contribution of around $-5\%$ at an unphysically heavy pion mass. Extending the FH relation to finite-momentum transfers, we also present calculations of the pion and nucleon electromagnetic form factors up to momentum transfers of around 7-8 GeV$^2$. Results for the nucleon are not able to confirm the existence of a sign change for the ratio $\frac{G_E}{G_M}$, but suggest that future calculations at lighter pion masses will provide fascinating insight into this behaviour at large momentum transfers.

==> standard_preamble.tex <==

\makeatletter
\@ifclassloaded{beamer}
{
  \usecolortheme[named=orange]{structure}
  \useoutertheme{infolines}
  \usetheme{Madrid}
  \setbeamertemplate{items}[default]
  \setbeamertemplate{blocks}[rounded][shadow=false]
  \setbeamertemplate{navigation symbols}{}

  %\let\oldhl\hl
  %\renewcommand\hl[1]
  %{%
	%\let\set@color\beamerorig@set@color
	%\let\reset@color\beamerorig@reset@color
	%\oldhl{#1}
  %}
  \newcommand{\gap}{\\~\\}
  \newcommand{\heading}[1]{{\large \textbf{#1}}}
  \newcommand{\importantpoint}[1]{
	\begin{center}
	  \alert{\large \textbf{#1}}
	\end{center}
  }
  \newcommand{\attseeker}[1]{{\large \textbf{#1}} }


}
{}
\makeatother

\newcommand{\usepackageifexists}[1]{\IfFileExists{#1.sty}{%
    \usepackage{#1}}{}}

\usepackageifexists{subfiles}
\usepackageifexists{amsmath}
\usepackageifexists{multirow}
\usepackageifexists{mathtools}
\usepackageifexists{graphicx}
\usepackageifexists{color}
\usepackageifexists{soul}
\usepackageifexists{epstopdf}
\usepackageifexists{simplewick}
\usepackageifexists{amssymb}

\graphicspath{{.}{graphics/}}

\newcommand{\vecp}[1]{\vec{#1}\mkern2mu\vphantom{#1}'}
\newcommand{\vecs}[1]{\vec{#1} \, ^2}
\newcommand{\vecps}[1]{\vec{#1}\mkern2mu\vphantom{#1}' \, ^2}

\newcommand{\Lagrangian}[0]{\mathcal{L}}

\newcommand{\eqcomma}[0]{\, ,}
\newcommand{\eqstop}[0]{\, .}

\newcommand{\eq}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\fig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\tab}[1]{Table \ref{tab:#1}}
\renewcommand{\sec}[1]{Sec.~\ref{sec:#1}}

\renewcommand{\d}[1]{\mathrm{d} #1 \,}
\newcommand{\dc}[1]{\mathrm{d}^3 #1 \,}

\newcommand{\half}{\frac{1}{2}}
\newcommand{\sone}{spin-$1$ }
\newcommand{\shalf}{spin-$\half$ }
\newcommand{\szero}{spin-$0$}
\newcommand{\bra}[1]{\langle \, #1 \, | \,}
\newcommand{\ket}[1]{\, | \, #1  \, \rangle}
\newcommand{\atlarget}{\xrightarrow{\text{large } t}}
\newcommand{\atlargedt}{\xrightarrow{\text{large } \Delta t}}
\newcommand{\bravac}{\bra{\Omega}}
\newcommand{\ketvac}{\ket{\Omega}}

\newcommand{\order}[1]{\mathcal{O}\left(#1\right)}

\renewcommand{\st}{\textsuperscript{st} }

\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\newcommand{\I}{\mathbb{I}}

\newcommand{\phm}{\phantom{-}}



\DeclareMathOperator{\Tr}{Tr}

